Provably efficient RL with Rich Observations via Latent State Decoding

We study the exploration problem in episodic MDPs with rich observations generated from a small number of latent states. Under certain identifiability assumptions, we demonstrate how to estimate a mapping from the observations to latent states inductively through a sequence of regression and clustering steps -- where previously decoded latent states provide labels for later regression problems -- and use it to construct good exploration policies. We provide finite-sample guarantees on the quality of the learned state decoding function and exploration policies, and complement our theory with an empirical evaluation on a class of hard exploration problems. Our method exponentially improves over $Q$-learning with na\"ive exploration, even when $Q$-learning has cheating access to latent states.

==> additional_exp.tex <==
Here we study the output of our algorithm to test whether it matches the theory.
In our experiment, we test $d = 5$ and $H=10$.
We use linear function class and set $N_{exp} = N_{id} = 1000$.
When $h \ge 2$, for $s_2$ there are 3 ways of getting there, and for $s_1$ there is only one way, so the underlying true linear regressor is \begin{align*}
	B = \begin{pmatrix}
	0.1 & 0 & 0 & \ldots& 0 \\
	0 & 1/30 & 0 &\ldots & 0 \\
	0 & 1/30 & 0 &\ldots & 0 \\
	0 & 1/30 & 0 &\ldots & 0 \\ 
	\end{pmatrix}.
\end{align*} 
To see this, note if  $x \sim E(s_1)$, \begin{align*}
	Bx = \begin{pmatrix}
	0.1 & 0 & 0 &  \ldots& 0 \\
	0 & 1/30 & 0 &\ldots & 0 \\
	0 & 1/30 & 0  &\ldots & 0 \\
	0 & 1/30 & 0  &\ldots & 0 \\ 
	\end{pmatrix} \begin{pmatrix}
	10\\
	0\\
	?\\
	...\\
	?
	\end{pmatrix} = \begin{pmatrix}
	1\\
	0 \\
	0\\
	0
	\end{pmatrix}
\end{align*} which is exactly $P(s,a|s_1)$.
Similarly if $x\sim E(s_2)$, we have \begin{align*}
Bx = \begin{pmatrix}
0.1 & 0 & 0 &  \ldots& 0 \\
0 & 1/30 & 0 &\ldots & 0 \\
0 & 1/30 & 0  &\ldots & 0 \\
0 & 1/30 & 0  &\ldots & 0 \\ 
\end{pmatrix} \begin{pmatrix}
0\\
10\\
?\\
...\\
?
\end{pmatrix} = \begin{pmatrix}
0\\
1/3 \\
1/3\\
1/3
\end{pmatrix}
\end{align*} which is $P(s,a|s_2)$.
We sampled some learned $\hat{g}_h$.

$\hat{g}_3$:\begin{verbatim}
0.0968    0.0008    0.0005    0.0002   -0.0000
-0.0004    0.0334    0.0013   -0.0223   -0.0056
-0.0008    0.0325    0.0119    0.0337    0.0287
0.0013    0.0338   -0.0141   -0.0106   -0.0248
\end{verbatim}

$\hat{g}_7$:\begin{verbatim}
0.0970   -0.0001   -0.0062    0.0029    0.0028
0.0000    0.0309   -0.0210    0.0183   -0.0203
0.0011    0.0358    0.0148   -0.0102    0.0078
0.0002    0.0330    0.0056   -0.0078    0.0100
\end{verbatim}

$\hat{g}_{10}$: \begin{verbatim}
0.0972    0.0003    0.0031    0.0005    0.0006
-0.0004    0.0353   -0.0153   -0.0110   -0.0040
-0.0000    0.0319    0.0189    0.0039    0.0180
-0.0008    0.0326   -0.0045    0.0059   -0.0158
\end{verbatim}

\simon{What other things should we show?}


\subsection{Stochastic Contextual Combination Lock}
\label{sec:stoc_comb_lock}
We next consider a hard stochastic problem, stochastic contextual combination lock.
There are two actions, $a$ and $b$.
There is only one state at $h=0$, $\states_0 = \left\{s_0\right\}$.
There are two states at $h=1$, $\states_1 = \left\{s_1,s_2\right\}$.
The transition rule at level $h=0$ is $P(\cdot|s_0,a) = \left[0.9,0.1\right]$ and $P(\cdot|s_1,a) = \left[0.1,0.9\right]$.

For $h \ge 2$, there are 3 states $\states_h = \left\{s_1,s_2,s_3\right\}$.
$s_3$ is the dead-end state, i.e., $P(\cdot|s_3,a) = P(\cdot|s_3,b) = [0,0,1]$.
The transition probability at $s_1$ is $P(\cdot|s_1,a) = [0.9,0.1,0]$  and $P(\cdot|s_1,b) = [0,0,1]$.
The transition probability at $s_2$ is $P(\cdot|s_2,a) = [0,0,1]$  and $P(\cdot|s_2,b) = [0.1,0.9,0]$.
At $s_1$, $a$ is the right action and at $s_2$, $b$ is the right action.
Therefore, we need to decode the state otherwise we cannot choose the right action.

We generate the context according the following rules.
If $s=s_1$, the first 3 coordinates are fixed $x_1 = 10$, $x_2 = 0$, $x_3=0$  and remaining ones are random $x_{4:d} \sim Bern(0.5)$, if $s=s_2$, the first 3 coordinates are fixed $x_1 = 0$, $x_2 = 10$, $x_3 = 10$  and remaining ones are random $x_{4:d} \sim Bern(0.5)$ and if $s=s_3$, the first 3 coordinates are fixed $x_1 = 0$, $x_2 = 0$, $x_3 = 10$  and remaining ones are random $x_{4:d} \sim Bern(0.5)$. 

\subsubsection{Study of Our Algorithm}
In our experiment, we test $d=5$, $H=10$.
We use linear function class and set $N_{exp} = 10000$, $N_{id}=100$, $N_{p}=10000$.
When $h \ge 2$, note there are $6$ state action pairs $(s_1,a)$, $(s_1,b)$, $(s_2,a)$, $(s_2,b)$, $(s_3,a)$, $(s_1,b)$.
With uniform exploration strategy, the underlying true regressor has the following form:\begin{align*}
B = \begin{pmatrix}
0.09 & 0.01 & 0 & 0 & \ldots & 0 \\
0 & 0 & 0.025 & 0 &\ldots & 0 \\
0 & 0 & 0.025 & 0 & \ldots & 0 \\
0.01 & 0.09 & 0 & 0 & \ldots & 0 \\
0 & 0 & 0.025 & 0 & \ldots & 0\\
0 &0 & 0.025 & 0 & \ldots & 0\\
\end{pmatrix}.
\end{align*} 
To see this if $x \sim E(s_1)$, \begin{align*}
	Bx = \begin{pmatrix}
	0.09 & 0.01 & 0 & 0 & \ldots & 0 \\
	0 & 0 & 0.025 & 0 &\ldots & 0 \\
	0 & 0 & 0.025 & 0 & \ldots & 0 \\
	0.01 & 0.09 & 0 & 0 & \ldots & 0 \\
	0 & 0 & 0.025 & 0 & \ldots & 0\\
	0 &0 & 0.025 & 0 & \ldots & 0\\
	\end{pmatrix} \begin{pmatrix}
	10\\
	0 \\
	0 \\
	? \\
	\ldots\\
	?
	\end{pmatrix} = \begin{pmatrix}
	0.9\\
	0 \\
	0 \\
	0.1 \\
	0 \\
	0 \\
	0
	\end{pmatrix} 
\end{align*} which is exactly $P(\cdot,\cdot|s_1)$.
We can check other conditional probability as well.

In this experiment, we test whether we can learn good $g_h$ and transition probability $\hat{P}$.
We sample some $\hat{g}_h$.

$\hat{g}_3$: \begin{verbatim}
0.0902    0.0096    0.0000    0.0025   -0.0009
0.0000    0.0000    0.0256    0.0057   -0.0009
0.0000    0.0000    0.0250    0.0044    0.0004
-0.0000   -0.0000    0.0243   -0.0075    0.0026
-0.0000   -0.0000    0.0251   -0.0026   -0.0021
0.0098    0.0904   -0.0000   -0.0025    0.0009
\end{verbatim}

$\hat{g}_7$: \begin{verbatim}
0.0000    0.0000    0.0252    0.0020    0.0037
0.0107    0.0913    0.0000    0.0021   -0.0017
-0.0000   -0.0000    0.0246   -0.0027   -0.0016
-0.0000    0.0000    0.0245    0.0059    0.0003
0.0893    0.0087   -0.0000   -0.0021    0.0017
-0.0000   -0.0000    0.0257   -0.0052   -0.0024
\end{verbatim}

$\hat{g}_{10}$: \begin{verbatim}
0.0000    0.0000    0.0250   -0.0046    0.0045
-0.0000   -0.0000    0.0250    0.0062   -0.0073
0.0890    0.0104   -0.0000    0.0015   -0.0019
0.0000   -0.0000    0.0246   -0.0061   -0.0010
-0.0000    0.0000    0.0254    0.0045    0.0039
0.0110    0.0896    0.0000   -0.0015    0.0019
\end{verbatim}

Note the order may not match because we don't observe the state directly, the order is based on we learned.

We also report the estimated transition probability.
For each state we report three matrix, each representing $P(\cdot|s,\cdot)$ for $s=s_1,s_2,s_3$.
Each row represents an action.

$\hat{P}_3:$
\begin{verbatim}
1     0     0
1     0     0

1.0000         0         0
0    0.9080    0.0920

0    0.0959    0.9041
1.0000         0         0
\end{verbatim}

$\hat{P}_7:$
\begin{verbatim}
1     0     0
1     0     0

0    0.9065    0.0935
1.0000         0         0

1.0000         0         0
0    0.0869    0.9131
\end{verbatim}


$\hat{P}_{10}:$
\begin{verbatim}
0     1     0
0     1     0

0    1.0000         0
0.0988         0    0.9012

0.8943         0    0.1057
0    1.0000         0
\end{verbatim}

==> comp.tex <==
\subsection{Connection with Q-learning}
Here we show how to construct a function class $G$ for prediction based on function class $F$ for $Q$ function.
Fix level $h \in 0,\ldots,H-1$. Suppose we know $Q(x',a) \in F$ where $x' \in \contexts_{h+1}$ and $F$ is some function class.
We also assume immediate reward $r(x',a) \in F$.
Consider the vector \begin{align*}
	v_{s'} = \begin{pmatrix}
	Q(x',a_1) - r(x',a_1) \\
	\ldots \\
	Q(x',a_K) - r(x',a_K) 
	\end{pmatrix} \in \mathbb{R}^K
\end{align*} with $s' \in \states_{h+1}$.
Note though this vector is defined through context, it is independent of the specific context.
To this see, notice that \begin{align*}
Q(x',a) - R(x',a) = Q(s,a) \triangleq \sum_{s'' \in \states{h+2}}P(s''|s',a) \expect_{x'' \in E(s'')}\left[\max_{a}Q(x'',a)\right].
\end{align*}
We view $v_{s'}$ as the representation of the hidden states $s'$.

Recall our oracle.
Given a rolling policy $\pi$, which induced a distribution over $(s,a) \in \states_{h} \times \actions$.
Let $D$ be this distribution, we want to predict $u_{s'}\triangleq P^{D}(\cdot,\cdot|s') \in \mathbb{R}^{\abs{\states_{h}}K}$ for $s' \in \states_{h+1}$.
Thus we only need to find a map $h^\pi$ that satisfies \begin{align*}
	h^\pi (v_s') = u_{s'} \text{ for all} s' \in \states_{h+1}.
\end{align*}
Note we have $\abs{\states_{h+1}}$ constraints
If $K \ge \abs{\states_{h+1}}$, we can find a linear map for $h^\pi$ with some identifiability condition because it suffices to show
\begin{align*}
\begin{pmatrix}
u_{s_1'} & \ldots & u_{s_{\abs{\states_{h+1}}}'}
\end{pmatrix} = A^\pi\begin{pmatrix}
v_{s_1'} & \ldots & v_{s_{\abs{\states_{h+1}}}'} \in \mathbb{R}^{\abs{\states_{h+1}}K \times K}
\end{pmatrix}.
\end{align*} for some $A^\pi \in \mathbb{R}^{\abs{\states_{h+1}}K \times K}$.
There are totally $\abs{\states_{h}}\times k \times \abs{\states_{h+1}}$ equations.
We have $\abs{\states_{h}}\times K \times K$ variables (dimension of $A^\pi$).
Thus in general we require $K \ge \abs{\states_{h+1}}$.

If $K < \abs{\states_{h+1}}$, $h^\pi$ needs to be non-linear.
A one layer ReLU network can make it.

\paragraph{Comparison with \cite{dann2018polynomial}} \cite{dann2018polynomial} only presented computationally efficient algorithm for deterministic transition dynamics.
Here we significantly relax this condition to non-degenerate stochastic transition matrix.


==> conclusion.tex <==
\subsection{Future Directions in Theory}
\paragraph{Minimax Regret Bounds}

\subsection{Future Direction in Methodology}
\paragraph{Combine with Imitation Learning}


\paragraph{Combine with Hierarchical RL}


\paragraph{More Advanced Search Algorithm}
A*-search?

\paragraph{Combine with Q-Learning}

==> dp.tex <==
See Algorithm~\ref{algo:dynamic} for the pseudo-code of dynamic programming, which computes the policy that maximizes reaching probability to a target state given the transition model as input. 
\begin{algorithm}[t]
	\floatname{algorithm}{Algorithm}
	\caption{Dynamics Programming}
	\label{algo:dynamic}
	\begin{algorithmic}[1]
		\Statex \textbf{Input}:Transition probabilities $P_1,\ldots,P_H$, target state $s^* \in \states_H$
		\Statex \textbf{Output}: Policy $\psi: \states_h \rightarrow \actions$.
		\State Define $V_H \in \mathbb{R}^{\abs{\states_H}}$ with $V_H(s^*) = 1$ and $V_H(s') = 0 $ for $s \neq s^*$.
		\For{$h = H-1,H-2,\ldots,0$}
			\For{$s \in \states_h$}
					\State $\psi(s) = \max_{a \in \actions} P_{h+1}(s,a)^\top V_{h+1}$ \alekh{$P_h$ and not $P_{h+1}$, right?}
					\simon{According to Algorithm~\ref{algo:stochastic} we should use $P_{h+1}$ because $P_{h+1}(s,a;s')$ for $s' \in \states_{h+1}$.}
					\State $V_h(s) = P_h(s,\psi(s))^\top V_{h+1}$
			\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm} 

==> justification.tex <==
Here we give an example showing that without Assumption~\ref{asmp:lower_bounded_reaching_prob}, the error can propagate exponentially. \nan{Why is this a justification for Assumption~\ref{asmp:lower_bounded_reaching_prob}?}
\simon{because this sample relies on the fact that $P(s_2) = \epsilon$ and $\epsilon$ can be arbitrarily small.}
\begin{example}
At a level $h-1$, suppose there are two states $s_1$ and $s_2$ and suppose for any policy $P(s_1) = 1-\epsilon$ and $P(s_2) = \epsilon$.
At level $h$ there are two states $s_1'$ and $s_2'$.
There are two actions $\actions = \left\{a,b\right\}$.
The transition probability $P(s_1'|\cdot,\cdot)$ is 
\begin{align*}
\begin{pmatrix}
\frac{1-3\epsilon}{1-\epsilon} & \frac{\alpha}{\alpha+\epsilon}\\
\frac{3\epsilon+3\alpha-1}{\epsilon+\alpha} & \frac{\alpha}{\alpha+\epsilon}
\end{pmatrix}
\end{align*}
and the transition probability $P(s_2'|\cdot,\cdot)$ is 
\begin{align*}
\begin{pmatrix}
\frac{2\epsilon}{1-\epsilon} & \frac{\epsilon}{\alpha+\epsilon}\\
\frac{1-2\epsilon-2\alpha}{\epsilon+\alpha} & \frac{\epsilon}{\alpha+\epsilon}
\end{pmatrix}
\end{align*} where the first row represents $s_1$, the second row represent $s_2$, the first column represents action  $a$ and the second column represents $b$ and we decide $\alpha$ later.

Now suppose our decoding function cannot differentiate $s_1$ and $s_2$ and these two states collapse into one learned state $\hat{s}$.
The transition probability from $\hat{s}$ to $s_1'$ is then \begin{align*}
\begin{pmatrix}
\frac{\alpha}{\epsilon+\alpha} & \frac{\alpha}{\epsilon+\alpha}
\end{pmatrix}
\end{align*}
and the transition probability from $\hat{s}$ to $s_2'$ is 
\begin{align*}
\begin{pmatrix}
\frac{\epsilon}{\epsilon+\alpha} & \frac{\epsilon}{\epsilon+\alpha}
\end{pmatrix}
\end{align*}
where the first column represents action $a$ and the second column represents action $b$.
Thus, it is impossible to distinguish $s_1'$ and $s_2'$.
Notice $\mu(s_2') \ge 2\epsilon$.
Thus the error can propagate exponentially. \nan{Why? What is the full construction for $H$ steps?}
\simon{This construction is quite informal. We can discuss whether we should add this example in our final version.}
Lastly, notice that we can choose $\alpha = \frac{5-5\epsilon}{12}$ to make the transition probabilities positive.
\end{example}

==> notation_table.tex <==
\begin{table}[tb]
	\centering
%	\resizebox{\columnwidth}{!}{%
		\renewcommand{\arraystretch}{1.5}
		\begin{tabular}{ |c|c|}
			\hline
			$\states_h$ & The set of true hidden states at level $h$, a subset of $[M]$. \\
			\hline
			$\widehat{S}_h$ & The set of learned hidden state at level $h$.\\
			\hline
			$s_h$ & A particular true hidden state at level $h$.\\
			\hline
			$\contexts$ & Context space at level $h$. \\
			\hline
			$\actions$ & Actions. \\
			\hline
			$E$ & Emission process, takes a hidden state and output a distribution over context.\\
			\hline
			$\pi$ & A policy that maps a context $x$ and the level $h$ into an action $a$.\\
			\hline
			$\prob^\pi(\cE)$ & given policy $\pi$, the probability that event $\cE$ happens.\\			\hline
			$\widehat{\prob}^\pi(\cE)$ & Estimated probability that given policy $\pi$, the  event $\cE$ happens.\\
			\hline
			 $\mu(s)$ & maximum reaching probability to $s$.\\
			 \hline
			 $\pi_s^*$ & The policy the maximizes the probability getting to state $s$.\\
			 \hline
			 $\nu$ & A distribution over $\states \times \actions$ or $\widehat{\states} \times \actions$.\\
			 \hline
			 $P(s,a;s')$  & Transition probability starting from $s_h$, taking action $a$ and gets to $s_{h+1}$.\\
			 \hline
			 $P^\nu(\hat{s},a;s')$  & Transition probability  given a distribution $\nu$ over $\widehat{\states} \times \actions$.\footnote{For learned states, the conditional probability may not be Markov.}\\
			 \hline
			 $P(s,a)$ & An $\abs{S_{h+1}}$ dimensional transition probability vector  starting from $s_h$, taking action $a$.\\
			 \hline
			 $Q_\nu$ & The induced distribution over $(s,a,s',x')$ or $(\hat{s},a,s',x')$ given a distribution $\nu$.\\
			 \hline
			 $\dataset$ & A data set. \\
			 \hline
			 $\phi_h$ & Embedding function  $\states_h \rightarrow \mathbb{R}^{MK}$.\\
			\hline
			$B_\nu(s';s,a)$& Backward probability, the conditional visited $(s,a)$ given $s'$ and a distribution over  $\states_{h} \times \actions$, $\nu$.\\
			\hline
			$B_\nu(s')$& An $\abs{\states_{h}}K$-dimensional vector where $(s,a)$ index representing $B_\nu(s';s,a)$.\\
			\hline
			$\gamma$ & Separation.\\
			\hline
		\end{tabular}
%	}
	\caption{Environment notations. Some time the subscript is omitted if it is clear.
		\label{tab:notation_table}
	}
\end{table}


\begin{table}[tb]
	\centering
	%	\resizebox{\columnwidth}{!}{%
	\renewcommand{\arraystretch}{1.5}
	\begin{tabular}{ |c|c|}
		\hline
			$\hat{s}_h$ & A particular learned hidden state at level $h$. \\
			\hline
			$\widehat{S}_h$ & The set of learned hidden state at level $h$.\\
			\hline
			$\hat{\nu}$ &  Estimation of  probability distribution over $\widehat{\states} \times \actions$.\\
			\hline
			$\hat{g}_h$ & Mapping from $\contexts$ to $R^{MK}$ (embedding space).\\
			\hline
			$\hat{f}_h$ & Mapping from the context to $\widehat{S}_h$ \\
			\hline
			$\pi_{\hat{s}}$ & Estimated policy that maximizes the probability of getting to $\hat{s}$.\\
			\hline
			$\widehat{P}(s_h,a;s')$  & Estimated transition probability starting from $s_h$, taking action $a$ and gets to $s_{h+1}$.\\
			\hline
			$\widehat{P}(s,a)$ & An $\abs{S_{h+1}}$ dimensional estimated transition probability vector  starting from $s_h$, taking action $a$.\\
			\hline
			$\widehat{B}_\nu(s';\hat{s},a)$& Backward probability, the conditional visited $(\hat{s},a) \in \widehat{\states}_{h} \times \actions$ given $s'$.\\
			\hline
			$\widehat{B}_\nu(s')$& An $\abs{\widehat{\states}_{h}}K$-dimensional vector where $(\hat{s},a)$ index representing $\widehat{B}_\nu(s';\hat{s},a)$.\\
			\hline
			$\pi_h$ & Exploration strategy for the $h$-th level.\\
			\hline
			$\tilde{\pi}$ & A policy that maps a learned $\hat{s}_{h}$ and level $h$ to an action. \\
			\hline
%			$\widehat{P}(\hat{s}_{h}|\hat{s}_{h-1},a)$ & Estimated probability from $\hat{s}_{h-1}$, taking action $a$ and gets to $\hat{s}_h$.\\
%			  \simon{Should we just abuse the notation}
%			\hline
%			 $\widehat{P}(\cdot|\hat{s}_h,a)$ & An $\abs{\widehat{S}_h}$ dimensional transition probability vector  starting from $s_h$, taking action $a$.\\
%			 \hline
			 $\alpha$ & The bijection that maps $\hat{s}_h$ to the corresponding $s_h$.\\
			 \hline
%			 $\Phi$ & Permutation matrix that maps the learned states to the true states.\\
			 \hline
	\end{tabular}
	%	}
	\caption{Notations used in the algorithms. Some time the subscript is omitted if it is clear.
%		\simon{
%			Should we just abuse the notation for bounding $\widehat{P}(\cdot|\hat{s}_h,a) - P(\cdot|\alpha(\hat{s}_h),a)$? We can make a order for $\widehat{P}(\cdot|\hat{s}_h,a)$ the same order as $P(\cdot|s,a)$
%			}
		\label{tab:notation_table_2}
	}
\end{table}

==> rel.tex <==
In this section we review some closely related works.

\cite{azizzadenesheli2016reinforcement} used spectral method to learn the best reactive policy for general POMDPs in the infinite horizon setting.
However, there are several drawbacks.
First, they only considered stochastic policy, i.e., for any context, the probability of taking any action has lower bounded probability (Page 8)
The optimal policy may not belong to this class.
Second, they assumed the ergodicity of any policy in the stochastic policy class they considered and their bounds depend on the mixing time (Page 8 assumption 1).
These two assumptions may be avoidable at least in the finite horizon problem.
Their bounds also depend on the number of observations.
This assumption may be unavoidable unless we have other assumptions.

The follow-up work \cite{azizzadenesheli2016contextual} considered the contextual POMDP. They still rely on stochastic policy and ergodicity assumptions.
Though asymptotically their bounds do not depend on the number of observations, the burn-in stage still require number of samples proportional to that.


\cite{oh2018self} proposed self-imitation learning.
The basic idea is that even for random policy there is some chance to get positive reward and we should imitate these good random policy.
Given the replay buffer $D = \left\{\left(s_t,a_t,R_t\right)\right\}$, they consider the loss function \begin{align*}
\expect_{s,a,R \in D}\left[-\log \pi_\theta\left(a|s\right)(R-V_\theta(s))_++\frac{1}{2}\norm{\left(R-V_\theta (s) \right)_+}_2^2\right].
\end{align*}
The use of ReLU encourages the agent to learn the good policy.


\cite{bellemare2016unifying} and the follow-up work~\cite{ostrovski2017count} adopt a past idea: count-based exploration~\citep{strehl2005theoretical,strehl2004empirical}.
For a state $x_t$, the main idea is to build a conditional probability distribution \[
\rho_n(x) = \rho (X_{n+1}=x|X_1\ldots X_n = x_{1:n}).
\]
and the pseudo-count is defined as $\hat{N}_n(x) = \hat{n}\rho_n (x)$ where $\hat{n}$ is the pseudo-count total $\hat{n}$.
They used a bonus of the form \[
R_n^+(x,a) = \beta (\hat{N}_n (x)+0.01)^{-1/2}
\] to represent the exploration bonus.
\cite{bellemare2016unifying} used CTS model~\citep{bellemare2014skip} and \cite{ostrovski2017count} used PixelCNN as density model.

